Auto-Instruct: Automatic Instruction Generation and Ranking for Black-Box Language Models

Large language models (LLMs) can perform a wide range of tasks by following natural language instructions, without the necessity of task-specific fine-tuning. Unfortunately, the performance of LLMs is greatly influenced by the quality of these instructions, and manually writing effective instructions for each task is a laborious and subjective process. In this paper, we introduce Auto-Instruct, a novel method to automatically improve the quality of instructions provided to LLMs. Our method leverages the inherent generative ability of LLMs to produce diverse candidate instructions for a given task, and then ranks them using a scoring model trained on a variety of 575 existing NLP tasks. In experiments on 118 out-of-domain tasks, Auto-Instruct surpasses both human-written instructions and existing baselines of LLM-generated instructions. Furthermore, our method exhibits notable generalizability even with other LLMs that are not incorporated into its training process.

==> Tables/main_results_present.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t]
\centering
% \setlength{\tabcolsep}{1.3mm}{
% \resizebox{0.9\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc@{}}
\toprule
\multicolumn{1}{l|}{\multirow{2}{*}{\textbf{Methods}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Generation}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Ranking}}} & \multicolumn{2}{c|}{\textbf{\textit{Few-shot}}}                          & \multicolumn{2}{c}{\textbf{\textit{Zero-shot}}}                                    \\
\multicolumn{1}{c|}{}   & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{}           & \textbf{\ SuperNI\ }                   & \textbf{\ BBH\ }                        & \textbf{\ SuperNI\ }  & \textbf{\ BBH\ }                                \\ \midrule
Empty Instruction*    & None & None                  & 57.03 & 51.18 &                 35.86            & 45.12                              \\
Human Instruction*     & Human & None                & 60.94                     & 50.30                      & {46.81}   & 45.59                              \\
Random Selection\dag     & LLM & Random             & 61.61                     & 50.88                      & {45.80}   & 45.98                              \\

iPrompt*            & LLM & Examples                      &   61.13    &   50.82    & -                           &      -                              \\
Auto-Instruct\dag          & LLM & Trained Model            & \textbf{64.35}                     & \textbf{52.04}                      & \textbf{49.50}              & \textbf{47.35} \\ \bottomrule
\end{tabular}
\end{table*}
